Prompting in the Wild: An Empirical Study of Prompt Evolution in Software Repositories

The adoption of Large Language Models (LLMs) is reshaping software development as developers integrate these LLMs into their applications. In such applications, prompts serve as the primary means of interacting with LLMs. Despite the widespread use of LLM-integrated applications, there is limited understanding of how developers manage and evolve prompts. This study presents the first empirical analysis of prompt evolution in LLM-integrated software development. We analyzed 1,262 prompt changes across 243 GitHub repositories to investigate the patterns and frequencies of prompt changes, their relationship with code changes, documentation practices, and their impact on system behavior. Our findings show that developers primarily evolve prompts through additions and modifications, with most changes occurring during feature development. We identified key challenges in prompt engineering: only 21.9% of prompt changes are documented in commit messages, changes can introduce logical inconsistencies, and misalignment often occurs between prompt changes and LLM responses. These insights emphasize the need for specialized testing frameworks, automated validation tools, and improved documentation practices to enhance the reliability of LLM-integrated applications.

==> 05-discussion.tex <==
\section{Discussion}
\label{sec:discussion}
% 
%IA: I am commenting this para. Move/merge the following two para into results. Prompts represent a unique and emerging type of software artifact that fundamentally differs from traditional components like code, documentation, or comments \cite{}. Through our empirical analysis of 1,262 prompt changes across 243 repositories, we examined how developers evolve and maintain prompts in practice, investigating their modification patterns, documentation practices, and the challenges that may appear in the prompt engineering process. Our analysis reveals significant gaps in current prompt evolution practices, particularly in testing, documentation, and validation of prompt changes. Based on our empirical analysis, we identify several key implications for both practitioners and researchers.

% \textbf{Documentation and Change Management:} The current state of prompt documentation practices is concerning, with only 21.9\% of prompt changes being explicitly documented in the commit messages and most of them being overly general. While traditional code documentation focuses on explaining implementation details \cite{},  'prompt documentation must capture both intended behavior and potential impacts on LLM responses. Practitioners should prioritize developing more comprehensive documentation practices that clearly articulate the reasoning behind prompt changes and their expected impacts. For researchers, this presents an opportunity to extend existing automatic commit message generation tools \cite{liu2020atom, nie2021coregen, dong2022fira}, which currently focus on code changes, to incorporate prompt modifications. These tools should be capable of analyzing prompt changes and generating meaningful commit messages that capture both the nature of the changes and their intended effects on LLM behavior\cite{}.

% \textbf{Testing and Validation Infrastructure:} Our findings reveal critical gaps in testing and validation practices for LLM-integrated systems, evidenced by only 7 out of 101 projects having suitable test cases and the frequent occurrence of logical inconsistencies in prompt modifications. Unlike traditional software where unit tests can validate specific functionality \cite{}, prompts require new testing approaches that can account for their natural language nature and the non-deterministic behavior of LLMs \cite{}. For practitioners, this suggests an immediate need to establish both testing protocols and systematic review processes specifically designed for prompts. For researchers, this opens opportunities to develop automated validation frameworks that can effectively validate prompt behavior while accounting for LLMs’ non-deterministic nature \cite{}. Such frameworks should focus on both functional correctness and the detection of potential issues in the natural language texts of a prompt before deployment.

% These findings underscore the need for both practical solutions and longer-term research initiatives to address the unique challenges of prompt engineering in LLM-integrated systems. As these systems become more prevalent in software development, addressing these challenges will be crucial for ensuring their reliability and maintainability.

==> tables/ablation_table.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}


% \usepackage{multirow}


\begin{table*}
\caption{The Result of Ablation Study}
\label{tab:ablation_result}
\centering
\begin{adjustbox}{max width=\textwidth}
\scriptsize
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}       & \multicolumn{4}{c|}{\textbf{ChatGPT}}       & \multicolumn{4}{c|}{\textbf{Gemini Pro}}    & \multicolumn{4}{c|}{\textbf{GPT-4}}         & \multicolumn{4}{c|}{\textcolor{blue}{\textbf{Starcoder2-Instruct}}} & \multicolumn{4}{c|}{\textcolor{blue}{\textbf{Overall Average}}} & \multicolumn{4}{l}{\textcolor{blue}{\textbf{Difference (Compared to Base)}}}  \\ 
\cline{2-25}\textcolor{blue}
{}                        & \textbf{ACC} & \textbf{TPR} & \textbf{TNR} & \textbf{AVG\_F1} & \textbf{ACC} & \textbf{TPR} & \textbf{TNR} & \textbf{AVG\_F1} & \textbf{ACC} & \textbf{TPR} & \textbf{TNR} & \textbf{AVG\_F1} & \textcolor{blue}{\textbf{ACC}} & \textcolor{blue}{\textbf{TPR}} & \textcolor{blue}{\textbf{TNR}} & \textcolor{blue}{\textbf{AVG\_F1}} & \textcolor{blue}{\textbf{ACC}} & \textcolor{blue}{\textbf{TPR}} & \textcolor{blue}{\textbf{TNR}} & \textcolor{blue}{\textbf{AVG\_F1}} & \textcolor{blue}{\textbf{ACC}} & \textcolor{blue}{\textbf{TPR}} & \textcolor{blue}{\textbf{TNR}} & \textcolor{blue}{\textbf{AVG\_F1}} \\ 
\hline
\textbf{Base AST Code Embedding} & 89.88 & 91.76 & 88.33 & 89.80   & 73.35 & 85.30 & 64.02 & 72.97   & 82.25 & 83.48 & 81.11 & 82.10   & \textcolor{blue}{85.40} & \textcolor{blue}{85.79} & \textcolor{blue}{84.96} & \textcolor{blue}{85.33}   & \textcolor{blue}{82.72} & \textcolor{blue}{86.59} & \textcolor{blue}{79.61} & \textcolor{blue}{82.55}        & -     & -     & -     & -                          \\ 
\hline
\textbf{Uniform Method Names}    & 88.36  & 92.89  & 85.07  & 88.33   & 75.30  & 88.93  & 64.78  & 74.97   & 80.90  & 82.56  & 79.59  & 80.83   & \textcolor{blue}{87.22} & \textcolor{blue}{90.05} & \textcolor{blue}{84.33} & \textcolor{blue}{87.20}   & \textcolor{blue}{82.95} & \textcolor{blue}{88.61} & \textcolor{blue}{78.44} & \textcolor{blue}{82.83}        & \textcolor{blue}{0.22}  & \textcolor{blue}{2.02}  & \textcolor{blue}{-1.17} & \textcolor{blue}{0.29}                       \\ 
\hline
\textbf{Uniform Variable Names}  & 85.49  & 87.80  & 83.49  & 85.40   & 75.07  & 85.35  & 67.06  & 74.56   & 83.52  & 86.66  & 80.51  & 83.39   & \textcolor{blue}{85.39} & \textcolor{blue}{88.73} & \textcolor{blue}{81.95} & \textcolor{blue}{85.34}   & \textcolor{blue}{82.37} & \textcolor{blue}{87.14} & \textcolor{blue}{78.25} & \textcolor{blue}{82.17}        & \textcolor{blue}{-0.36} & \textcolor{blue}{0.55}  & \textcolor{blue}{-1.36} & \textcolor{blue}{-0.38}                      \\ 
\hline
\textbf{No Comment Line}         & 83.98  & 86.21  & 81.58  & 83.43   & 73.29  & 83.79  & 64.56  & 72.68   & 78.03  & 79.99  & 75.38  & 77.37   & \textcolor{blue}{81.49} & \textcolor{blue}{83.95} & \textcolor{blue}{78.97} & \textcolor{blue}{81.45}   & \textcolor{blue}{79.20} & \textcolor{blue}{83.49} & \textcolor{blue}{75.12} & \textcolor{blue}{78.73}        & \textcolor{blue}{-3.53} & \textcolor{blue}{-3.10} & \textcolor{blue}{-4.49} & \textcolor{blue}{-3.82}                      \\
\hline
\end{tabular}
\end{adjustbox}
\end{table*}

% \begin{table*}
% \caption{The Result of Ablation Study}
% \label{tab:ablation_result}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
% \hline
% \multirow{2}{*}{}                & \multicolumn{4}{c|}{\textbf{ChatGPT}}                               & \multicolumn{4}{c|}{\textbf{Gemini Pro }}                           & \multicolumn{4}{c|}{\textbf{GPT-4 }}                                & \multicolumn{4}{c|}{\textbf{Overall Average}}                       & \multicolumn{4}{c}{\textbf{Difference (Compared to Base)}}    \\ 
% \cline{2-21}
%                                  & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC} & \textbf{TPR} & \textbf{TNR} & \textbf{AVG\_F1}  \\ 
% \hline
% \textbf{Base AST Code Embedding} & \textbf{89.88} & 91.76          & \textbf{88.34} & \textbf{89.80}   & 73.36          & 85.30          & 64.02          & 72.97            & 82.26          & 83.49          & \textbf{81.12} & 82.10            & \textbf{81.83} & 86.85          & \textbf{77.83} & \textbf{81.62}   & -            & -            & -            & -                 \\ 
% \hline
% \textbf{Uniform Method Names}    & 88.36          & \textbf{92.89} & 85.07          & 88.33            & \textbf{75.30} & \textbf{88.93} & 64.78          & \textbf{74.97}   & 80.90          & 82.56          & 79.59          & 80.83            & 81.52          & \textbf{88.13} & 76.48          & 81.38            & -0.31         & +1.27        & -1.34         & -0.24              \\ 
% \hline
% \textbf{Uniform Variable Names}  & 85.49          & 87.80          & 83.49          & 85.40            & 75.07          & 85.35          & \textbf{67.06} & 74.56            & \textbf{83.52} & \textbf{86.66} & 80.51          & \textbf{83.39}   & 81.36          & 86.60          & 77.02          & 81.12            & -0.47         & +0.25         & -0.80         & -0.51              \\ 
% \hline
% \textbf{No Comment Line}         & 83.98          & 86.21          & 81.58          & 83.43            & 73.29          & 83.79          & 64.56          & 72.68            & 78.03          & 79.99          & 75.38          & 77.37            & 78.43          & 83.33          & 73.84          & 77.83            & -3.40         & -3.52         & -3.99         & -3.80              \\
% \hline
% \end{tabular}
% }
% \end{table*}

==> tables/aigc_detectors_table.tex <==

% \usepackage{graphicx}
% \usepackage{multirow}

% \usepackage{multirow}


% \usepackage{multirow}

% \usepackage{multirow}


\begin{table*}
\centering
\caption{Performance of Existing AIGC Detectors (Default Temperature)}
\label{tab:aigc1}
\begin{adjustbox}{max width=\textwidth}
\scriptsize
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}             & \multicolumn{4}{c|}{\textbf{ChatGPT}}                         & \multicolumn{4}{c|}{\textbf{Gemini Pro}}                      & \multicolumn{4}{c|}{\textbf{GPT-4}}                           & \multicolumn{4}{c|}{\textbf{\textcolor{blue}{Starcoder2-Instruct} }}            & \multicolumn{4}{c}{\textbf{\textcolor{blue}{Mean of Every Datasets}}}            \\ 
\cline{2-21}
                              & \textbf{ACC} & \textbf{TPR} & \textbf{TNR} & \textbf{AVG\_F1} & \textbf{ACC} & \textbf{TPR} & \textbf{TNR} & \textbf{AVG\_F1} & \textbf{ACC} & \textbf{TPR} & \textbf{TNR} & \textbf{AVG\_F1} & \textbf{\textcolor{blue}{ACC}} & \textbf{\textcolor{blue}{TPR}} & \textbf{\textcolor{blue}{TNR}} & \textbf{\textcolor{blue}{AVG\_F1}} & \textbf{\textcolor{blue}{ACC}} & \textbf{\textcolor{blue}{TPR}} & \textbf{\textcolor{blue}{TNR}} & \textbf{\textcolor{blue}{AVG\_F1}}  \\ 
\hline
\textbf{GPT2 Output Detector} & 45.61        & 0.00         & 100.00       & 31.88            & 36.66        & 0.00         & 100.00       & 34.54            & 46.65        & 49.07        & 53.07        & 32.25            & \textcolor{blue}{50.22}        & \textcolor{blue}{26.49}        & \textcolor{blue}{73.95}        & \textcolor{blue}{45.54}            & \textcolor{blue}{48.86}        & \textcolor{blue}{18.89}        & \textcolor{blue}{81.75}        & \textcolor{blue}{36.05}             \\ 
\hline
\textbf{DetectGPT}            & 46.44        & 2.95         & 100.00       & 33.61            & 38.97        & 7.21         & 99.51        & 39.13            & 43.71        & 43.31        & 52.26        & 37.24            & \textcolor{blue}{52.64}        & \textcolor{blue}{7.26}         & \textcolor{blue}{98.01}        & \textcolor{blue}{39.70}            & \textcolor{blue}{48.99}        & \textcolor{blue}{15.18}        & \textcolor{blue}{87.45}        & \textcolor{blue}{37.42}             \\ 
\hline
\textbf{Sapling}              & 55.17        & 94.46        & 11.60        & 44.10            & 33.79        & 92.73        & 7.83         & 37.25            & 45.90        & 43.62        & 35.09        & 35.55            & \textcolor{blue}{52.18}        & \textcolor{blue}{47.49}        & \textcolor{blue}{56.88}        & \textcolor{blue}{50.81}            & \textcolor{blue}{49.97}        & \textcolor{blue}{69.57}        & \textcolor{blue}{27.85}        & \textcolor{blue}{41.93}             \\ 
\hline
\textbf{GPTZero}              & 53.13        & 85.00        & 0.83         & 35.22            & 45.34        & 100.00       & 0.00         & 31.16            & 38.82        & 39.65        & 29.85        & 34.98            & \textcolor{blue}{53.87}        & \textcolor{blue}{28.74}        & \textcolor{blue}{79.00}        & \textcolor{blue}{47.39}            & \textcolor{blue}{47.83}        & \textcolor{blue}{63.35}        & \textcolor{blue}{27.42}        & \textcolor{blue}{37.19}             \\ 
\hline
\textbf{GLTR}                 & 44.53        & 48.73        & 44.64        & 41.63            & 41.83        & 45.32        & 68.46        & 47.80            & 51.83        & 45.48        & 46.59        & 46.59            & \textcolor{blue}{47.21}        & \textcolor{blue}{47.08}        & \textcolor{blue}{47.34}        & \textcolor{blue}{44.22}            & \textcolor{blue}{50.83}        & \textcolor{blue}{46.65}        & \textcolor{blue}{51.76}        & \textcolor{blue}{45.06}             \\
\hline
\end{tabular}
\end{adjustbox}
\end{table*}

% \begin{table*}
% \caption{Performance of Existing AIGC Detectors (Default Temperature)}
% \label{tab:aigc1}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
% \hline
% \multirow{2}{*}{}    & \multicolumn{4}{c|}{\textbf{ChatGPT}}     & \multicolumn{4}{c|}{\textbf{Gemini Pro}}   & \multicolumn{4}{c|}{\textbf{GPT-4}}      & \multicolumn{4}{c}{\textbf{Mean of Every Datasets}}  \\ 
% \cline{2-17}
%                      & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}    & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}    & \textbf{TNR}    & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1}              \\ 
% \hline
% GPT2 Output Detector & 45.61 & 0.00  & 100.00 & 31.88   & 36.66 & 0.00   & 100.00 & 34.54   & 46.65 & 49.07 & 53.07 & 32.25   & 48.41 & 16.36 & 84.36 & 32.89                \\ 
% \hline
% DetectGPT            & 46.44 & 2.95  & 100.00 & 33.61   & 38.97 & 7.21   & 99.51  & 39.13   & 43.71 & 43.31 & 52.26 & 37.24   & 47.78 & 17.82 & 83.92 & 36.66                \\ 
% \hline
% Sapling              & 55.17 & 94.46 & 11.60  & 44.10   & 33.79 & 92.73  & 7.83   & 37.25   & 45.90 & 43.62 & 35.09 & 35.56   & 49.23 & 76.93 & 18.17 & 38.97                \\ 
% \hline
% GPTZero              & 53.13 & 85.00 & 0.83   & 35.22   & 45.34 & 100.00 & 0.00   & 31.16   & 38.82 & 39.65 & 29.85 & 34.98   & 45.82 & 74.88 & 10.23 & 33.79                \\ 
% \hline
% GLTR                 & 44.53 & 48.73 & 44.64  & 41.63   & 41.83 & 45.32  & 68.46  & 47.80   & 51.83 & 45.48 & 51.74 & 46.59   & 52.04 & 46.51 & 54.94 & 45.34                \\ 
% \hline
% \end{tabular}
% }
% \end{table*}

%GPTSniffer           & 55.87 & 16.67 & 100.00 & 43.11   & 54.59 & 14.29  & 89.52  & 38.91   & 45.72 & 43.00 & 51.98 & 43.46   & 52.06 & 24.65 & 80.50 & 41.83                \\

==> tables/collected_features_table.tex <==
% \usepackage{graphicx}


\begin{table}
\centering
\caption{Collected Source Code Features}
\label{tab:features}

\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l|l} 
\hline
\textbf{Features}                                                                      & \textbf{Definitions}                                                                                                                                          \\ 
\hline
SumCyclomatic                                                                          & \begin{tabular}[c]{@{}l@{}}Sum of cyclomatic complexity \\ of all nested functions or methods.\end{tabular}                                              \\ 
\hline
AvgCountLineCode                                                                       & \begin{tabular}[c]{@{}l@{}}Average number of lines contai-\\ -ning source code for all nested\\ functions or methods.\end{tabular}                            \\ 
\hline
CountLineCodeDecl                                                                      & \begin{tabular}[c]{@{}l@{}}Number of lines containing decl-\\ -arative source code\end{tabular}                                                               \\ 
\hline
CountDeclFunction                                                                      & Number of functions                                                                                                                                           \\ 
\hline
MaxNesting                                                                             & \begin{tabular}[c]{@{}l@{}}Maximum nesting level of (if, w-\\ -hile, for, switch etc.)\end{tabular}                                                           \\ 
\hline
CountLineBlank                                                                         & Number of blank lines                                                                                                                                         \\ 
\hline
Keywords                                                                               & \begin{tabular}[c]{@{}l@{}}The ratio between the number of \\ language keyword tokens to the \\ number of total tokens\end{tabular}                           \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Operators in if, else, \\ and while statements\end{tabular} & \begin{tabular}[c]{@{}l@{}}The ratio between the number of \\ operators in if, else, and while sta-\\ -tements to the number of total \\ tokens\end{tabular}  \\
\hline
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/components.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|p{2.8cm}|p{5.2cm}|}
\hline
\textbf{Component} & \textbf{Definition} \\
\hline
Role & Assigns a specific role or persona to the model to guide its response. \\
\hline
Directive & Describes what the LLM is supposed to do by providing instructions or questions to specify the desired task. \\
\hline
Example & Offers sample inputs/outputs to demonstrate expected behavior. \\
\hline
Output Instruction & Specifies how the response should be formatted and styled. \\
\hline
Consideration & Commands that provide guidance to ensure the model adheres to specific requirements. \\
\hline
Additional Information & Supplies extra context and background information to enhance relevance and specificity. \\
\hline
\end{tabular}
\caption{Categories and Definitions of Prompt Components}
\label{tab:component-definitions}
\end{table}


==> tables/cosine_similarity.tex <==
% \begin{table}
% \centering
% \caption{Cosine Similarity and P-Value Between Code Embeddings of AI-generated and Human-written Code (Default Temperature)}
% \label{tab:emb_cossim}
% \begin{adjustbox}{max width=\textwidth}
% \scriptsize
% \begin{tabular}{l|l|l|l|l} 
% \hline
%                                       & \multicolumn{1}{c|}{\textcolor{blue}{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{\textcolor{blue}{\textbf{Gemini Pro}}} & \multicolumn{1}{c|}{\textcolor{blue}{\textbf{GPT-4}}} & \multicolumn{1}{c}{\textcolor{blue}{\textbf{Starcoder2-Instruct}}}  \\ 
% \hline
% \textcolor{blue}{\textbf{Cosine Similarity}}     & \textcolor{blue}{73.87}                                 & \textcolor{blue}{\textbf{77.58}}                                     & \textcolor{blue}{76.56}                               & \textcolor{blue}{75.20}                                    \\ 
% \hline
% \textcolor{blue}{\textbf{P-Value}}     & \textcolor{blue}{0.2180}                                 & \textcolor{blue}{\textbf{0.5428}}                                     & \textcolor{blue}{0.2800}                               & \textcolor{blue}{0.1750}                                    \\ 
% \hline
% \end{tabular}
% \end{adjustbox}
% \end{table}

% \begin{table}
% \centering
% \caption{Cosine Similarity Between Embeddings of AI-generated and Human-written Code (Default Temperature)}
% \label{tab:emb_cossim}
% \begin{adjustbox}{max width=\textwidth}
% \tiny
% \begin{tabular}{l|l|l|l|l} 
% \hline
%                                       & \multicolumn{1}{c|}{\textbf{ChatGPT}} & \multicolumn{1}{c|}{\textbf{Gemini Pro}} & \multicolumn{1}{c|}{\textbf{GPT-4}} & \multicolumn{1}{c}{\textbf{Starcoder2}}  \\ 
% \hline
% \textbf{Cosine Similarity-Code}     & 92.07                                 & \textbf{96.70}                                     & 95.01                               & 92.73                                    \\ 
% \hline
% \textbf{Cosine Similarity-AST}      & 96.03                                 & \textbf{98.08}                                    & \textbf{98.08}                               & 97.13                                    \\ 
% \hline
% \textbf{Cosine Similarity-Code+AST} & 92.80                                  & \textbf{96.95}                                    & 96.02                               & 93.96                                    \\
% \hline
% \end{tabular}
% \end{adjustbox}
% \end{table}

==> tables/gptsniffer_table_tempdef.tex <==
% \usepackage{graphicx}

\begin{table}
\centering
\caption{The Evaluation Of GPTSniffer On Our Datasets (Default Temperature)}
\label{tab:sniffer1}
\begin{adjustbox}{max width=\textwidth}
\tiny
\begin{tabular}{l|l|l|l|l} 
\hline
\textbf{Dataset-Generation LLM-Language} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1}  \\ 
\hline
MBPP-ChatGPT-Python                      & 44.85          & 0.00           & 100.00         & 30.96             \\ 
\hline
MBPP-Gemini Pro-Python                   & 49.23          & 0.00           & 100.00         & 32.99             \\ 
\hline
MBPP-GPT-4-Python                        & 47.69          & 0.00           & 100.00         & 32.29             \\ 
\hline
\textcolor{blue}{MBPP-Starcoder2-Instruct-Python}                   & \textcolor{blue}{72.95}          & \textcolor{blue}{52.04}          & \textcolor{blue}{93.87}          & \textcolor{blue}{71.72}             \\ 
\hline
HumanEval-ChatGPT-Python                 & 60.61          & 0.00           & 100.00         & 37.74             \\ 
\hline
HumanEval-ChatGPT-Java                   & 32.26          & 0.00           & 100.00         & 24.39             \\ 
\hline
HumanEval-ChatGPT-C++                    & 100.00         & 100.00         & 100.00         & 100.00            \\ 
\hline
HumanEval-Gemini Pro-Python              & 54.55          & 0.00           & 100.00         & 35.30             \\ 
\hline
HumanEval-Gemini Pro-Java                & 65.62          & 0.00           & 100.00         & 39.63             \\ 
\hline
HumanEval-Gemini Pro-C++                 & 60.61          & 85.71          & 42.11          & 60.02             \\ 
\hline
HumanEval-GPT-4-Python                   & 54.55          & 0.00           & 100.00         & 35.30             \\ 
\hline
HumanEval-GPT-4-Java                     & 57.58          & 0.00           & 100.00         & 36.54             \\ 
\hline
HumanEval-GPT-4-C++                      & 96.97          & 95.00          & 100.00         & 96.87             \\ 
\hline
\textcolor{blue}{HumanEval-Starcoder2-Instruct-Python}              & \textcolor{blue}{50.00}          & \textcolor{blue}{0.00}           & \textcolor{blue}{100.00}         & \textcolor{blue}{33.34}             \\ 
\hline
\textcolor{blue}{HumanEval-Starcoder2-Instruct-Java}                & \textcolor{blue}{50.00}          & \textcolor{blue}{0.00}           & \textcolor{blue}{100.00}         & \textcolor{blue}{33.34}             \\ 
\hline
\textcolor{blue}{HumanEval-Starcoder2-Instruct-C++}                 & \textcolor{blue}{85.29}          & \textcolor{blue}{100.00}         & \textcolor{blue}{70.58}          & \textcolor{blue}{84.96}             \\ 
\hline
CodeSearchNet-ChatGPT-Python             & 50.00          & 0.00           & 100.00         & 33.34             \\ 
\hline
CodeSearchNet-ChatGPT-Java               & 47.50          & 0.00           & 100.00         & 32.21             \\ 
\hline
CodeSearchNet-Gemini Pro-Python          & 50.00          & 0.00           & 100.00         & 33.34             \\ 
\hline
CodeSearchNet-Gemini Pro-Java            & 47.50          & 0.00           & 95.00          & 32.21             \\ 
\hline
CodeSearchNet-GPT-4-Python               & 50.00          & 0.00           & 100.00         & 33.34             \\ 
\hline
CodeSearchNet-GPT-4-Java                 & 35.90          & 0.00           & 93.33          & 26.42             \\ 
\hline
\textcolor{blue}{CodeSearchNet-Starcoder2-Instruct-Python}          & \textcolor{blue}{57.50}          & \textcolor{blue}{30.00}          & \textcolor{blue}{85.00}          & \textcolor{blue}{54.02}             \\ 
\hline
\textcolor{blue}{CodeSearchNet-Starcoder2-Instruct-Java}            & \textcolor{blue}{52.50}          & \textcolor{blue}{30.00}          & \textcolor{blue}{75.00}          & \textcolor{blue}{49.96}             \\ 
\hline
\textcolor{blue}{\textbf{Average}}                         & \textcolor{blue}{\textbf{57.24}} & \textcolor{blue}{\textbf{20.53}} & \textcolor{blue}{\textbf{93.95}} & \textcolor{blue}{\textbf{45.01}}    \\
\hline
\end{tabular}
\end{adjustbox}
\end{table}

% \begin{table}
% \centering
% \caption{The Evaluation Of GPTSniffer On Our Datasets (Default Temperature)}
% \label{tab:sniffer1}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l|l|l|l|l} 
% \hline
% \textbf{Dataset-Generation LLM-Language} & \textbf{ACC} & \textbf{TPR} & \textbf{TNR} & \textbf{AVG\_F1}  \\ 
% \hline
% MBPP-ChatGPT-Python             & 44.85        & 0.00         & 100.00       & 30.96             \\ 
% \hline
% MBPP-Gemini Pro-Python          & 49.23        & 0.00         & 100.00       & 32.99             \\ 
% \hline
% MBPP-GPT-4-Python               & 47.69        & 0.00         & 100.00       & 32.29             \\ 
% \hline
% HumanEval-ChatGPT-Python        & 60.61        & 0.00         & 100.00       & 37.74             \\ 
% \hline
% HumanEval-ChatGPT-Java          & 32.26        & 0.00         & 100.00       & 24.39             \\ 
% \hline
% HumanEval-ChatGPT-C++           & 100.00       & 100.00       & 100.00       & 100.00            \\ 
% \hline
% HumanEval-Gemini Pro-Python     & 54.55        & 0.00         & 100.00       & 35.30             \\ 
% \hline
% HumanEval-Gemini Pro-Java       & 65.62        & 0.00         & 100.00       & 39.63             \\ 
% \hline
% HumanEval-Gemini Pro-C++        & 60.61        & 85.71        & 42.11        & 60.02             \\ 
% \hline
% HumanEval-GPT-4-Python          & 54.55        & 0.00         & 100.00       & 35.30             \\ 
% \hline
% HumanEval-GPT-4-Java            & 57.58        & 0.00         & 100.00       & 36.54             \\ 
% \hline
% HumanEval-GPT-4-C++             & 96.97        & 95.00        & 100.00       & 96.87             \\ 
% \hline
% CodeSearchNet-ChatGPT-Python    & 50.00        & 0.00         & 100.00       & 33.34             \\ 
% \hline
% CodeSearchNet-ChatGPT-Java      & 47.50        & 0.00         & 100.00       & 32.21             \\ 
% \hline
% CodeSearchNet-Gemini Pro-Python & 50.00        & 0.00         & 100.00       & 33.34             \\ 
% \hline
% CodeSearchNet-Gemini Pro-Java   & 47.50        & 0.00         & 95.00        & 32.21             \\ 
% \hline
% CodeSearchNet-GPT-4-Python      & 50.00        & 0.00         & 100.00       & 33.34             \\ 
% \hline
% CodeSearchNet-GPT-4-Java        & 35.90        & 0.00         & 93.33        & 26.42             \\ 
% \hline
% \textbf{Average}                         & \textbf{55.86}        & \textbf{15.60}        & \textbf{96.14}        & \textbf{41.83}             \\
% \hline
% \end{tabular}
% }
% \end{table}

==> tables/llm_table_temp0.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}


\begin{table*}
\caption{Performance of LLM-based Approaches (Temperature = 0)}
\label{tab:llm_result_temp0}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}                 & \multicolumn{4}{c|}{ChatGPT}    & \multicolumn{4}{c|}{Gemini Pro}  & \multicolumn{4}{c|}{GPT-4}      & \multicolumn{4}{c}{Mean of Every Dataset}  \\ 
\cline{2-17}
                                  & ACC   & TPR   & TNR   & AVG\_F1 & ACC   & TPR    & TNR   & AVG\_F1 & ACC   & TPR   & TNR   & AVG\_F1 & ACC   & TPR   & TNR   & AVG\_F1             \\ 
\hline
GPT-3.5 (Zero shot) - Code        & 51.73 & 99.84 & 0.00  & 33.74   & 46.16 & 100.00 & 0.00  & 31.42   & 50.43 & 98.73 & 0.00  & 33.40   & 49.44 & 99.52 & 0.00  & 32.85               \\ 
\hline
GPT-3.5 (In-context) - Code       & 51.48 & 83.23 & 20.13 & 44.56   & 40.99 & 64.91  & 20.53 & 37.66   & 53.00 & 82.58 & 22.73 & 47.14   & 48.49 & 76.91 & 21.13 & 43.12               \\ 
\hline
GPT-3.5 (Fine-tuned) - Code       & 82.67 & 94.75 & 70.63 & 81.33   & 62.10 & 95.92  & 34.98 & 56.85   & 81.24 & 99.21 & 64.00 & 78.15   & 75.34 & 96.63 & 56.54 & 72.11               \\ 
\hline
GPT-3.5 (Zero shot) - AST         & 43.78 & 68.85 & 15.31 & 37.18   & 47.13 & 73.88  & 24.67 & 42.43   & 45.66 & 62.73 & 27.84 & 41.46   & 45.52 & 68.49 & 22.61 & 40.36               \\ 
\hline
GPT-3.5 (In-context) - AST        & 52.43 & 83.75 & 20.92 & 45.90   & 43.59 & 69.56  & 19.87 & 39.47   & 57.74 & 83.04 & 31.31 & 53.30   & 51.25 & 78.78 & 24.03 & 46.22               \\ 
\hline
GPT-3.5 (Fine-tuned) - AST        & 70.69 & 76.37 & 64.44 & 68.67   & 63.10 & 74.93  & 50.55 & 59.11   & 65.09 & 70.17 & 62.63 & 62.09   & 66.29 & 73.82 & 59.21 & 63.29               \\ 
\hline
GPT-3.5 (Zero shot) - Code + AST  & 50.98 & 96.19 & 1.25  & 34.27   & 46.23 & 98.60  & 1.70  & 32.85   & 50.58 & 97.90 & 1.43  & 34.68   & 49.26 & 97.56 & 1.46  & 33.93               \\ 
\hline
GPT-3.5 (In-context) - Code + AST & 50.93 & 53.68 & 43.60 & 46.32   & 41.80 & 55.37  & 28.99 & 38.65   & 52.65 & 66.27 & 37.73 & 49.35   & 48.46 & 58.44 & 36.77 & 44.77               \\ 
\hline
GPT-3.5 (Fine-tuned) - Code + AST & 75.48 & 85.36 & 61.29 & 70.99   & 62.54 & 79.66  & 50.14 & 59.51   & 82.77 & 96.15 & 69.80 & 80.45   & 73.60 & 87.06 & 60.41 & 70.31               \\
\hline
\end{tabular}
}
\end{table*}

==> tables/llm_table_tempdef.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}


\begin{table*}
\caption{Performance of LLM-based Approaches (Default Temperature)}
\label{tab:llm_result_temp_def}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}                 & \multicolumn{4}{c|}{ChatGPT}    & \multicolumn{4}{c|}{Gemini Pro} & \multicolumn{4}{c|}{GPT-4}       & \multicolumn{4}{c}{Mean of Every Dataset}  \\ 
\cline{2-17}
                                  & ACC   & TPR   & TNR   & AVG\_F1 & ACC   & TPR   & TNR   & AVG\_F1 & ACC   & TPR    & TNR   & AVG\_F1 & ACC   & TPR   & TNR   & AVG\_F1             \\ 
\hline
GPT-3.5 (Zero shot) - Code        & 52.64 & 99.90 & 2.57  & 36.60   & 51.67 & 99.81 & 0.09  & 34.10   & 54.15 & 100.00 & 0.05  & 35.11   & 52.82 & 99.90 & 0.90  & 35.27               \\ 
\hline
GPT-3.5 (In-context) - Code       & 51.71 & 81.31 & 18.50 & 44.51   & 41.19 & 66.64 & 18.01 & 37.20   & 55.58 & 83.80  & 25.76 & 49.80   & 49.49 & 77.25 & 20.76 & 43.83               \\ 
\hline
GPT-3.5 (Fine-tuned) - Code       & 82.18 & 89.13 & 77.24 & 81.79   & 70.41 & 82.23 & 60.81 & 68.60   & 88.89 & 93.33  & 84.18 & 88.22   & 80.49 & 88.23 & 74.08 & 79.54               \\ 
\hline
GPT-3.5 (Zero shot) - AST         & 48.16 & 69.77 & 19.30 & 40.92   & 48.56 & 74.73 & 25.81 & 44.19   & 43.92 & 64.61  & 21.51 & 39.85   & 46.88 & 69.70 & 22.21 & 41.65               \\ 
\hline
GPT-3.5 (In-context) - AST        & 50.77 & 82.24 & 13.69 & 41.07   & 40.59 & 73.83 & 12.42 & 35.21   & 53.32 & 83.38  & 21.72 & 46.91   & 48.23 & 79.82 & 15.94 & 41.06               \\ 
\hline
GPT-3.5 (Fine-tuned) - AST        & 64.18 & 46.71 & 81.82 & 58.96   & 55.86 & 56.76 & 59.55 & 53.07   & 65.64 & 83.22  & 48.96 & 62.61   & 61.89 & 62.23 & 63.44 & 58.21               \\ 
\hline
GPT-3.5 (Zero shot) - Code + AST  & 55.50 & 97.78 & 4.29  & 38.78   & 44.65 & 97.54 & 0.69  & 31.30   & 52.05 & 98.19  & 1.77  & 35.51   & 50.73 & 97.84 & 2.25  & 35.20               \\ 
\hline
GPT-3.5 (In-context) - Code + AST & 46.27 & 50.71 & 40.43 & 42.90   & 37.90 & 52.01 & 22.01 & 32.70   & 52.57 & 61.81  & 43.50 & 50.25   & 45.58 & 54.84 & 35.31 & 41.95               \\ 
\hline
GPT-3.5 (Fine-tuned) - Code + AST & 75.25 & 91.68 & 57.12 & 72.57   & 63.06 & 85.23 & 44.26 & 59.37   & 75.37 & 90.42  & 61.87 & 71.72   & 71.23 & 89.11 & 54.42 & 67.89               \\
\hline
\end{tabular}
}
\end{table*}


==> tables/ml_table_temp0.tex <==
\begin{table*}
\caption{Performance of Machine Learning Classifier with Code Metrics (Temperature = 0)}
\label{tab:ml_result_temp0}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}           & \multicolumn{6}{c|}{ChatGPT}                    & \multicolumn{6}{c}{Gemini Pro}                  \\ 
\cline{2-13}
                            & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1 & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1  \\ 
\hline
ML (RandomForestClassifier) & 82.07 & 83.95 & 78.75 & 82.41 & 79.04 & 80.73   & 66.84 & 72.72 & 64.93 & 65.15 & 67.29 & 66.22    \\ 
\hline
\multirow{2}{*}{}           & \multicolumn{6}{c|}{GPT-4}                      & \multicolumn{6}{c}{Mean of Every Dataset}       \\ 
\cline{2-13}
                            & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1 & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1  \\ 
\hline
ML (RandomForestClassifier) & 71.33 & 69.25 & 74.58 & 69.41 & 71.46 & 70.44   & 73.41 & 75.31 & 72.75 & 72.33 & 72.60 & 72.46    \\
\hline
\end{tabular}
}
\end{table*}

==> tables/ml_table_tempdef.tex <==
\begin{table*}
\caption{Performance of Machine Learning Classifier with Code Metrics (Default Temperature)}
\label{tab:ml_result_tempdef}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}               & \multicolumn{6}{c|}{ChatGPT}                    & \multicolumn{6}{c}{Gemini Pro}                  \\ 
\cline{2-13}
                                & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1 & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1  \\ 
\hline
ML (GradientBoostingClassifier) & 78.72 & 84.81 & 73.62 & 80.43 & 76.14 & 78.28   & 72.78 & 81.10 & 65.89 & 72.69 & 72.14 & 72.41    \\ 
\hline
\multirow{2}{*}{}               & \multicolumn{6}{c|}{GPT-4}                      & \multicolumn{6}{c}{Mean of Averages}            \\ 
\cline{2-13}
                                & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1 & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1  \\ 
\hline
ML (GradientBoostingClassifier) & 76.03 & 78.82 & 72.52 & 76.04 & 75.09 & 75.57   & 75.84 & 81.58 & 70.68 & 76.38 & 74.46 & 75.42    \\
\hline
\end{tabular}
}
\end{table*}

==> tables/overall_table_temp0.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}


\begin{table*}
\centering
\caption{Overall Performance Comparison (Temperature = 0)}
\label{tab:overall_result_temp0}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}                              & \multicolumn{4}{c|}{\textbf{ChatGPT}}                               & \multicolumn{4}{c|}{\textbf{Gemini Pro}}                            & \multicolumn{4}{c|}{\textbf{GPT-4}}                                 & \multicolumn{4}{c}{\textbf{Overall Average}}                         \\ 
\cline{2-17}
                                               & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1}  \\ 
\hline
\textbf{ChatGPT (Fine-tuned) - Code}           & 82.67          & \textbf{94.75} & 70.63          & 81.33            & 62.10          & \textbf{95.92} & 34.98          & 56.85            & 81.24          & \textbf{99.21} & 64.00          & 78.15            & 75.34          & \textbf{96.63} & 56.54          & 72.11             \\ 
\hline
\textbf{ChatGPT (Fine-tuned) - AST}            & 70.69          & 76.37          & 64.44          & 68.67            & 63.10          & 74.93          & 50.55          & 59.11            & 65.09          & 70.17          & 62.63          & 62.09            & 66.29          & 73.82          & 59.21          & 63.29             \\ 
\hline
\textbf{ChatGPT (Fine-tuned) - Code + AST}     & 75.48          & 85.36          & 61.29          & 70.99            & 62.54          & 79.66          & 50.14          & 59.51            & 82.77          & 96.15          & 69.80          & 80.45            & 73.60          & 87.06          & 60.41          & 70.31             \\ 
\hline
\textbf{Code Metrics (RandomForestClassifier)} & 82.07          & 83.95          & 78.75          & 80.73            & 66.84          & 72.72          & 64.93          & 66.22            & 71.33          & 69.25          & 74.58          & 70.44            & 73.41          & 75.31          & 72.75          & 72.46             \\ 
\hline
\textbf{Code Embedding - Code}                 & 87.49          & 89.69          & \textbf{85.27} & 86.61            & 68.67          & 56.76          & \textbf{75.27} & 63.32            & 82.37          & 90.87          & 75.53          & 79.94            & 79.51          & 79.11          & \textbf{78.69} & 76.62             \\ 
\hline
\textbf{Code Embedding - AST}                  & \textbf{88.79} & 93.96          & 80.93          & \textbf{87.44}   & \textbf{72.63} & 82.73          & 64.56          & \textbf{72.25}   & 81.85          & 85.67          & 78.17          & 81.80            & \textbf{81.09} & 87.45          & 74.55          & \textbf{80.50}    \\ 
\hline
\textbf{Code Embedding - Code + AST}           & 86.65          & 88.16          & 82.93          & 85.34            & 63.10          & 66.95          & 60.14          & 62.91            & \textbf{84.48} & 85.56          & \textbf{83.71} & \textbf{84.41}   & 78.07          & 80.22          & 75.59          & 77.55             \\
\hline
\end{tabular}
}
\end{table*}

==> tables/overall_table_tempdef.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}


% \usepackage{graphicx}
% \usepackage{multirow}

% \usepackage{multirow}


\begin{table*}[ht]
\centering
\caption{Overall Performance Comparison - Within (Default Temperature)}
\label{tab:overall_result_tempdef}
\begin{adjustbox}{max width=\textwidth}
\scriptsize
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}             & \multicolumn{4}{c|}{\textbf{ChatGPT}}                                      & \multicolumn{4}{c|}{\textbf{Gemini Pro}}                                   & \multicolumn{4}{c|}{\textbf{GPT-4}}                                         & \multicolumn{4}{c|}{\textcolor{blue}{\textbf{Starcoder2-Instruct}}}                                   & \multicolumn{4}{c}{\textcolor{blue}{\textbf{Overall Average}}}                               \\ 
\cline{2-21}
                              & \textbf{ACC} & \textbf{TPR} & \textbf{TNR} & \textbf{AVG\_F1} & \textbf{ACC} & \textbf{TPR} & \textbf{TNR} & \textbf{AVG\_F1} & \textbf{ACC} & \textbf{TPR} & \textbf{TNR} & \textbf{AVG\_F1} & \textcolor{blue}{\textbf{ACC}} & \textcolor{blue}{\textbf{TPR}} & \textcolor{blue}{\textbf{TNR}} & \textcolor{blue}{\textbf{AVG\_F1}} & \textcolor{blue}{\textbf{ACC}} & \textcolor{blue}{\textbf{TPR}} & \textcolor{blue}{\textbf{TNR}} & \textcolor{blue}{\textbf{AVG\_F1}}  \\ 

\hline
\textcolor{blue}{\textbf{GPT-3.5 (Zero shot)-Code} }     & \textcolor{blue}{52.64} & \textcolor{blue}{\textbf{99.90}} & \textcolor{blue}{2.57}  & \textcolor{blue}{36.60} & \textcolor{blue}{51.67} & \textcolor{blue}{\textbf{99.81}} & \textcolor{blue}{0.09}  & \textcolor{blue}{34.10} & \textcolor{blue}{54.15} & \textcolor{blue}{\textbf{100.00}} & \textcolor{blue}{0.05}  & \textcolor{blue}{35.11} & \textcolor{blue}{52.11} & \textcolor{blue}{\textbf{99.93}} & \textcolor{blue}{0.68}  & \textcolor{blue}{34.78} & \textcolor{blue}{52.64} & \textcolor{blue}{\textbf{99.91}} & \textcolor{blue}{0.85}  & \textcolor{blue}{35.15}  \\ 
\hline
\textcolor{blue}{\textbf{GPT-3.5 (In-context)-Code}}     & \textcolor{blue}{51.71} & \textcolor{blue}{81.31}  & \textcolor{blue}{18.50} & \textcolor{blue}{44.51} & \textcolor{blue}{41.19} & \textcolor{blue}{66.64}  & \textcolor{blue}{18.01} & \textcolor{blue}{37.20} & \textcolor{blue}{55.58} & \textcolor{blue}{83.80}  & \textcolor{blue}{25.76} & \textcolor{blue}{49.80} & \textcolor{blue}{49.53} & \textcolor{blue}{80.21}  & \textcolor{blue}{18.12} & \textcolor{blue}{42.94} & \textcolor{blue}{49.50} & \textcolor{blue}{77.99}  & \textcolor{blue}{20.10} & \textcolor{blue}{43.61}  \\ 
\hline
\textbf{GPT-3.5 (Fine-tuned)-Code}     & 82.18 & 89.13  & 77.24 & 81.79 & 70.41 & 82.23  & 60.81 & 68.60 & \textbf{88.89} & 93.33  & \textbf{84.18} & \textbf{88.22} & \textcolor{blue}{82.98} & \textcolor{blue}{89.34}  & \textcolor{blue}{77.61} & \textcolor{blue}{82.26} & \textcolor{blue}{81.12} & \textcolor{blue}{88.51}  & \textcolor{blue}{74.96} & \textcolor{blue}{80.22}  \\ 
\hline
\textcolor{blue}{\textbf{GPT-3.5 (Zero shot)-AST}}       & \textcolor{blue}{48.16} & \textcolor{blue}{69.77}  & \textcolor{blue}{19.30} & \textcolor{blue}{40.92} & \textcolor{blue}{48.56} & \textcolor{blue}{74.73}  & \textcolor{blue}{25.81} & \textcolor{blue}{44.19} & \textcolor{blue}{43.92} & \textcolor{blue}{64.61}  & \textcolor{blue}{21.51} & \textcolor{blue}{39.85} & \textcolor{blue}{48.19} & \textcolor{blue}{70.53}  & \textcolor{blue}{25.90} & \textcolor{blue}{42.73} & \textcolor{blue}{47.21} & \textcolor{blue}{69.91}  & \textcolor{blue}{23.13} & \textcolor{blue}{41.92}  \\ 
\hline
\textcolor{blue}{\textbf{GPT-3.5 (In-context)-AST}}      & \textcolor{blue}{50.77} & \textcolor{blue}{82.24}  & \textcolor{blue}{13.69} & \textcolor{blue}{41.07} & \textcolor{blue}{40.59} & \textcolor{blue}{73.83}  & \textcolor{blue}{12.42} & \textcolor{blue}{35.21} & \textcolor{blue}{53.32} & \textcolor{blue}{83.38}  & \textcolor{blue}{21.72} & \textcolor{blue}{46.91} & \textcolor{blue}{49.19} & \textcolor{blue}{70.38}  & \textcolor{blue}{27.55} & \textcolor{blue}{42.47} & \textcolor{blue}{48.47} & \textcolor{blue}{77.46}  & \textcolor{blue}{18.85} & \textcolor{blue}{41.41}  \\ 
\hline
\textbf{GPT-3.5 (Fine-tuned)-AST}      & 64.18 & 46.71  & 81.82 & 58.96 & 55.86 & 56.76  & 59.55 & 53.07 & 65.64 & 83.22  & 48.96 & 62.61 & \textcolor{blue}{60.10} & \textcolor{blue}{53.50}  & \textcolor{blue}{68.20} & \textcolor{blue}{54.53} & \textcolor{blue}{61.44} & \textcolor{blue}{60.05}  & \textcolor{blue}{64.63} & \textcolor{blue}{57.29}  \\ 
\hline
\textcolor{blue}{\textbf{GPT-3.5 (Zero shot)-Code+AST}}  & \textcolor{blue}{55.50} & \textcolor{blue}{97.78}  & \textcolor{blue}{4.29}  & \textcolor{blue}{38.78} & \textcolor{blue}{44.65} & \textcolor{blue}{97.54}  & \textcolor{blue}{0.69}  & \textcolor{blue}{31.30} & \textcolor{blue}{52.05} & \textcolor{blue}{98.19}  & \textcolor{blue}{1.77}  & \textcolor{blue}{35.51} & \textcolor{blue}{52.56} & \textcolor{blue}{97.99}  & \textcolor{blue}{2.28}  & \textcolor{blue}{35.89} & \textcolor{blue}{51.19} & \textcolor{blue}{97.87}  & \textcolor{blue}{2.26}  & \textcolor{blue}{35.37}  \\ 
\hline
\textcolor{blue}{\textbf{GPT-3.5 (In-context)-Code+AST}} & \textcolor{blue}{46.27} & \textcolor{blue}{50.71}  & \textcolor{blue}{40.43} & \textcolor{blue}{42.90} & \textcolor{blue}{37.90} & \textcolor{blue}{52.01}  & \textcolor{blue}{22.01} & \textcolor{blue}{32.70} & \textcolor{blue}{52.57} & \textcolor{blue}{61.81}  & \textcolor{blue}{43.50} & \textcolor{blue}{50.25} & \textcolor{blue}{49.10} & \textcolor{blue}{59.15}  & \textcolor{blue}{38.30} & \textcolor{blue}{45.66} & \textcolor{blue}{46.46} & \textcolor{blue}{55.92}  & \textcolor{blue}{36.06} & \textcolor{blue}{42.88}  \\ 
\hline
\textbf{GPT-3.5 (Fine-tuned)-Code+AST} & 75.25 & 91.68  & 57.12 & 72.57 & 63.06 & 85.23  & 44.26 & 59.37 & 75.37 & 90.42  & 61.87 & 71.72 & \textcolor{blue}{67.09} & \textcolor{blue}{73.66}  & \textcolor{blue}{61.43} & \textcolor{blue}{61.79} & \textcolor{blue}{70.19} & \textcolor{blue}{85.25}  & \textcolor{blue}{56.17} & \textcolor{blue}{66.36}  \\ 
\hline
\textbf{Code Metrics (GB)}             & 78.72 & 84.81  & 73.62 & 78.28 & 72.78 & 81.10  & \textbf{65.89} & 72.41 & 76.03 & 78.82  & 72.52 & 75.57 & \textcolor{blue}{74.01} & \textcolor{blue}{80.86}  & \textcolor{blue}{67.02} & \textcolor{blue}{73.67} & \textcolor{blue}{75.84} & \textcolor{blue}{81.58}  & \textcolor{blue}{70.68} & \textcolor{blue}{74.98}  \\ 
\hline
\textbf{Code Embedding-Code}           & 81.15 & 83.37  & 80.41 & 80.91 & 68.12 & 78.50  & 60.27 & 67.87 & 81.76 & 84.20  & 79.90 & 81.47 & \textcolor{blue}{86.09} & \textcolor{blue}{86.21}  & \textcolor{blue}{\textbf{86.01}} & \textcolor{blue}{86.00} & \textcolor{blue}{79.28} & \textcolor{blue}{83.07}  & \textcolor{blue}{76.65} & \textcolor{blue}{79.06}  \\
\hline
\textbf{Code Embedding-AST}            & \textbf{89.89} & 91.76  & \textbf{88.34} & \textbf{89.80} & \textbf{73.36} & 85.30  & 64.02 & \textbf{72.97} & 82.26 & 83.49  & 81.12 & 82.10 & \textcolor{blue}{85.40} & \textcolor{blue}{85.79}  & \textcolor{blue}{84.96} & \textcolor{blue}{85.33} & \textcolor{blue}{\textbf{82.72}} & \textcolor{blue}{86.59}  & \textcolor{blue}{\textbf{79.61}} & \textcolor{blue}{\textbf{82.55}}  \\ 
\hline
\textbf{Code Embedding-Code+AST}      & 84.85 & 84.67  & 85.45 & 84.46 & 70.05 & 79.90  & 62.28 & 69.81 & 82.16 & 81.88  & 82.25 & 82.00 & \textcolor{blue}{\textbf{87.12}} & \textcolor{blue}{90.28}  & \textcolor{blue}{83.93} & \textcolor{blue}{\textbf{87.10}} & \textcolor{blue}{81.05} & \textcolor{blue}{84.18}  & \textcolor{blue}{78.48} & \textcolor{blue}{80.84}  \\
\hline
\end{tabular}
\end{adjustbox}
\end{table*}

% \begin{table*}
% \centering
% \caption{Overall Performance Comparison (Default Temperature)}
% \label{tab:overall_result_tempdef}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
% \hline
% \multirow{2}{*}{}                                 & \multicolumn{4}{c|}{\textbf{ChatGPT}}                               & \multicolumn{4}{c|}{\textbf{Gemini Pro}}                            & \multicolumn{4}{c|}{\textbf{GPT-4}}                                 & \multicolumn{4}{c}{\textbf{Overall Average}}                         \\ 
% \cline{2-17}
%                                                   & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1}  \\ 
% \hline
% \textbf{ChatGPT (Fine-tuned) - Code}              & 82.18          & 89.13          & 77.24          & 81.79            & 70.41          & 82.23          & 60.81          & 68.60            & \textbf{88.89} & \textbf{93.33} & \textbf{84.18} & \textbf{88.22}   & 80.49          & 88.23          & 74.08          & 79.54             \\ 
% \hline
% \textbf{ChatGPT (Fine-tuned) - AST}               & 64.18          & 46.71          & 81.82          & 58.96            & 55.86          & 56.76          & 59.55          & 53.07            & 65.64          & 83.22          & 48.96          & 62.61            & 61.89          & 62.23          & 63.44          & 58.21             \\ 
% \hline
% \textbf{ChatGPT (Fine-tuned) - Code + AST}        & 75.25          & 91.68          & 57.12          & 72.57            & 63.06          & 85.23          & 44.26          & 59.37            & 75.37          & 90.42          & 61.87          & 71.72            & 71.23          & \textbf{89.11} & 54.42          & 67.89             \\ 
% \hline
% \textbf{Code Metrics (GradienBoostingClassifier)} & 78.72          & 84.81          & 73.62          & 78.28            & 72.78          & 81.10          & \textbf{65.89} & 72.41            & 76.03          & 78.82          & 72.52          & 75.57            & 75.84          & 81.58          & 70.68          & 75.42             \\ 
% \hline
% \textbf{Code Embedding - Code}                    & 81.15          & 83.37          & 80.41          & 80.91            & 68.12          & 78.50          & 60.27          & 67.87            & 81.76          & 84.20          & 79.90          & 81.47            & 77.01          & 82.02          & 73.53          & 76.75             \\ 
% \hline
% \textbf{Code Embedding - AST}                     & \textbf{89.89} & \textbf{91.76} & \textbf{88.34} & \textbf{89.80}   & \textbf{73.36} & \textbf{85.30} & 64.02          & \textbf{72.97}   & 82.26          & 83.49          & 81.12          & 82.10            & \textbf{81.83} & 86.85          & \textbf{77.83} & \textbf{81.62}    \\ 
% \hline
% \textbf{Code Embedding - Code + AST}              & 84.85          & 84.67          & 85.45          & 84.46            & 70.05          & 79.90          & 62.28          & 69.81            & 82.16          & 81.88          & 82.25          & 82.00            & 79.02          & 82.15          & 76.66          & 78.76             \\
% \hline
% \end{tabular}
% }
% \end{table*}

==> tables/overall_table_tempdef_across.tex <==
% \usepackage{multirow}


\begin{table*}
\centering
\caption{Overall Performance Comparison - Across (Default Temperature)}
\label{tab:overall_result_tempdef_across}
\begin{adjustbox}{max width=\textwidth}
\scriptsize
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}                      & \multicolumn{4}{c|}{\textcolor{blue}{\textbf{ChatGPT }}}                        & \multicolumn{4}{c|}{\textcolor{blue}{\textbf{Gemini Pro }}}                     & \multicolumn{4}{c|}{\textcolor{blue}{\textbf{GPT-4 }}}                          & \multicolumn{4}{c|}{\textcolor{blue}{\textbf{Starcoder2-Instruct}}}                     & \multicolumn{4}{c}{\textcolor{blue}{\textbf{Overall Average}}}                   \\ 
\cline{2-21}
                                       & \textcolor{blue}{\textbf{ACC}} & \textcolor{blue}{\textbf{TPR}} & \textcolor{blue}{\textbf{TNR}} & \textcolor{blue}{\textbf{AVG\_F1}} & \textcolor{blue}{\textbf{ACC}} & \textcolor{blue}{\textbf{TPR}} & \textcolor{blue}{\textbf{TNR}} & \textcolor{blue}{\textbf{AVG\_F1}} & \textcolor{blue}{\textbf{ACC}} & \textcolor{blue}{\textbf{TPR}} & \textcolor{blue}{\textbf{TNR}} & \textcolor{blue}{\textbf{AVG\_F1}} & \textcolor{blue}{\textbf{ACC}} & \textcolor{blue}{\textbf{TPR}} & \textcolor{blue}{\textbf{TNR}} & \textcolor{blue}{\textbf{AVG\_F1}} & \textcolor{blue}{\textbf{ACC}} & \textcolor{blue}{\textbf{TPR}} & \textcolor{blue}{\textbf{TNR}} & \textcolor{blue}{\textbf{AVG\_F1}}  \\ 
\hline
\textcolor{blue}{\textbf{GPT-3.5 (In-context)-Code}}     & \textcolor{blue}{51.76}        & \textcolor{blue}{66.13}        & \textcolor{blue}{33.17}        & \textcolor{blue}{44.29}            & \textcolor{blue}{47.38}        & \textcolor{blue}{81.75}        & \textcolor{blue}{19.50}        & \textcolor{blue}{40.92}            & \textcolor{blue}{55.12}        & \textcolor{blue}{86.78}        & \textcolor{blue}{19.75}        & \textcolor{blue}{46.24}            & \textcolor{blue}{48.36}        & \textcolor{blue}{82.17}        & \textcolor{blue}{14.55}        & \textcolor{blue}{40.01}            & \textcolor{blue}{50.66}        & \textcolor{blue}{79.21}        & \textcolor{blue}{21.74}        & \textcolor{blue}{42.87}             \\ 
\hline
\textcolor{blue}{\textbf{GPT-3.5 (Fine-tuned)-Code}}     & \textcolor{blue}{52.11}        & \textcolor{blue}{56.50}        & \textcolor{blue}{45.63}        & \textcolor{blue}{44.80}            & \textcolor{blue}{50.64}        & \textcolor{blue}{72.27}        & \textcolor{blue}{34.30}        & \textcolor{blue}{43.44}            & \textcolor{blue}{53.26}        & \textcolor{blue}{49.10}        & \textcolor{blue}{54.55}        & \textcolor{blue}{46.01}            & \textcolor{blue}{51.26}        & \textcolor{blue}{12.98}        & \textcolor{blue}{89.53}        & \textcolor{blue}{37.61}            & \textcolor{blue}{51.82}        & \textcolor{blue}{47.71}        & \textcolor{blue}{56.00}        & \textcolor{blue}{42.96}             \\ 
\hline
\textcolor{blue}{\textbf{GPT-3.5 (In-context)-AST}}      & \textcolor{blue}{46.69}        & \textcolor{blue}{40.21}        & \textcolor{blue}{53.53}        & \textcolor{blue}{43.93}            & \textcolor{blue}{51.05}        & \textcolor{blue}{49.21}        & \textcolor{blue}{51.95}        & \textcolor{blue}{48.47}            & \textcolor{blue}{51.38}        & \textcolor{blue}{42.30}        & \textcolor{blue}{59.02}        & \textcolor{blue}{48.74}            & \textcolor{blue}{47.95}        & \textcolor{blue}{40.99}        & \textcolor{blue}{54.95}        & \textcolor{blue}{45.78}            & \textcolor{blue}{49.27}        & \textcolor{blue}{43.18}        & \textcolor{blue}{54.86}        & \textcolor{blue}{46.73}             \\ 
\hline
\textcolor{blue}{\textbf{GPT-3.5 (Fine-tuned)-AST}}      & \textcolor{blue}{52.77}        & \textcolor{blue}{39.29}        & \textcolor{blue}{64.67}        & \textcolor{blue}{44.33}            & \textcolor{blue}{51.17}        & \textcolor{blue}{47.87}        & \textcolor{blue}{53.49}        & \textcolor{blue}{46.27}            & \textcolor{blue}{51.47}        & \textcolor{blue}{60.54}        & \textcolor{blue}{40.53}        & \textcolor{blue}{44.67}            & \textcolor{blue}{52.93}        & \textcolor{blue}{30.49}        & \textcolor{blue}{75.51}        & \textcolor{blue}{39.75}            & \textcolor{blue}{52.09}        & \textcolor{blue}{44.55}        & \textcolor{blue}{58.55}        & \textcolor{blue}{43.76}             \\ 
\hline
\textcolor{blue}{\textbf{GPT-3.5 (In-context)-Code+AST}} & \textcolor{blue}{47.50}        & \textcolor{blue}{54.70}        & \textcolor{blue}{41.11}        & \textcolor{blue}{44.16}            & \textcolor{blue}{48.08}        & \textcolor{blue}{60.96}        & \textcolor{blue}{35.71}        & \textcolor{blue}{45.02}            & \textcolor{blue}{54.08}        & \textcolor{blue}{60.78}        & \textcolor{blue}{44.40}        & \textcolor{blue}{50.46}            & \textcolor{blue}{49.95}   \textcolor{blue} {}    & \textcolor{blue}{59.66}        & \textcolor{blue}{40.10}        & \textcolor{blue}{47.82}            & \textcolor{blue}{49.90}        & \textcolor{blue}{59.02}        & \textcolor{blue}{40.33}        & \textcolor{blue}{46.86}             \\ 
\hline
\textcolor{blue}{\textbf{GPT-3.5 (Fine-tuned)-Code+AST}} & \textcolor{blue}{51.72}        & \textcolor{blue}{51.55}        & \textcolor{blue}{49.57}        & \textcolor{blue}{46.32}            & \textcolor{blue}{52.64}        & \textcolor{blue}{71.98}        & \textcolor{blue}{34.70}        & \textcolor{blue}{45.42}            & \textcolor{blue}{54.48}        & \textcolor{blue}{56.08}        & \textcolor{blue}{51.90}        & \textcolor{blue}{48.72}            & \textcolor{blue}{51.54}        & \textcolor{blue}{29.68}        & \textcolor{blue}{73.50}        & \textcolor{blue}{45.47}            & \textcolor{blue}{52.59}        & \textcolor{blue}{52.32}        & \textcolor{blue}{52.42}        & \textcolor{blue}{46.48}             \\ 
\hline
\textcolor{blue}{\textbf{Code Metrics (GB)}}             & \textcolor{blue}{56.79}        & \textcolor{blue}{54.43}        & \textcolor{blue}{59.11}        & \textcolor{blue}{51.82}            & \textcolor{blue}{58.35}        & \textcolor{blue}{59.93}        & \textcolor{blue}{56.15}        & \textcolor{blue}{54.62}            & \textcolor{blue}{55.32}        & \textcolor{blue}{47.68}        & \textcolor{blue}{64.02}        & \textcolor{blue}{50.96}            & \textcolor{blue}{51.88}        & \textcolor{blue}{37.63}        & \textcolor{blue}{66.33}        & \textcolor{blue}{46.72}            & \textcolor{blue}{55.59}        & \textcolor{blue}{49.92}        & \textcolor{blue}{61.40}        & \textcolor{blue}{51.03}             \\ 
\hline
\textcolor{blue}{\textbf{Code Embedding-Code}}           & \textcolor{blue}{51.15}        & \textcolor{blue}{39.01}        & \textcolor{blue}{63.72}        & \textcolor{blue}{42.20}            & \textcolor{blue}{57.23}        & \textcolor{blue}{50.91}        & \textcolor{blue}{62.70}        & \textcolor{blue}{50.72}            & \textcolor{blue}{52.19}        & \textcolor{blue}{35.71}        & \textcolor{blue}{69.11}        & \textcolor{blue}{43.38}            & \textcolor{blue}{53.47}        & \textcolor{blue}{38.67}        & \textcolor{blue}{69.42}        & \textcolor{blue}{46.83}            & \textcolor{blue}{53.51}        & \textcolor{blue}{41.08}        & \textcolor{blue}{66.24}        & \textcolor{blue}{45.78}             \\ 
\hline
\textcolor{blue}{\textbf{Code Embedding-AST}}            & \textcolor{blue}{53.47}        & \textcolor{blue}{38.67}        & \textcolor{blue}{69.42}        & \textcolor{blue}{46.83}            & \textcolor{blue}{53.55}        & \textcolor{blue}{38.06}        & \textcolor{blue}{67.38}        & \textcolor{blue}{45.41}            & \textcolor{blue}{50.84}        & \textcolor{blue}{26.09}        & \textcolor{blue}{78.72}        & \textcolor{blue}{42.83}            & \textcolor{blue}{50.07}        & \textcolor{blue}{18.26}        & \textcolor{blue}{82.12}        & \textcolor{blue}{37.78}            & \textcolor{blue}{51.98}        & \textcolor{blue}{30.27}        & \textcolor{blue}{74.41}        & \textcolor{blue}{43.21}             \\ 
\hline
\textcolor{blue}{\textbf{Code Embedding-Code+AST}}       & \textcolor{blue}{54.85}        & \textcolor{blue}{42.37}        & \textcolor{blue}{67.89}        & \textcolor{blue}{46.64}            & \textcolor{blue}{55.27}        & \textcolor{blue}{45.83}        & \textcolor{blue}{64.11}        & \textcolor{blue}{48.42}            & \textcolor{blue}{55.94}        & \textcolor{blue}{37.82}        & \textcolor{blue}{74.49}        & \textcolor{blue}{47.58}            & \textcolor{blue}{49.09}        & \textcolor{blue}{17.31}        & \textcolor{blue}{81.06}        & \textcolor{blue}{38.36}            & \textcolor{blue}{53.79}        & \textcolor{blue}{35.83}        & \textcolor{blue}{71.89}        & \textcolor{blue}{45.25}             \\
\hline
\end{tabular}
\end{adjustbox}
\end{table*}

==> tables/within_vs_across_cossim.tex <==
\begin{table*}
\centering
\caption{Comparison on the Characteristics of Training and Testing dataset - Within vs. Across (Default Temperature)}
\label{tab:within_vs_across_cossim}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}                      & \multicolumn{2}{c|}{\textcolor{blue}{\textbf{ChatGPT }}} & \multicolumn{2}{c|}{\textcolor{blue}{\textbf{Gemini Pro }}} & \multicolumn{2}{c|}{\textcolor{blue}{\textbf{GPT-4 }}} & \multicolumn{2}{c|}{\textcolor{blue}{\textbf{Starcoder2-Instruct}}} & \multicolumn{2}{c}{\textcolor{blue}{\textbf{Overall Average }}}  \\ 
\cline{2-11}
                                       & \textcolor{blue}{\textbf{Within}} & \textcolor{blue}{\textbf{Across}}      & \textcolor{blue}{\textbf{Within}} & \textcolor{blue}{\textbf{Across}}         & \textcolor{blue}{\textbf{Within}} & \textcolor{blue}{\textbf{Across}}    & \textcolor{blue}{\textbf{Within}} & \textcolor{blue}{\textbf{Across}}         & \textcolor{blue}{\textbf{Within}} & \textcolor{blue}{\textbf{Across}}              \\ 
\hline
\textcolor{blue}{\textbf{Cosine Similarity of AST Embeddings}} & \textcolor{blue}{98.61}           & \textcolor{blue}{78.76}                & \textcolor{blue}{98.65}           & \textcolor{blue}{75.18}                   & \textcolor{blue}{98.63}           & \textcolor{blue}{78.09}              & \textcolor{blue}{98.85}           & \textcolor{blue}{79.46}                 & \textcolor{blue}{98.68}          & \textcolor{blue}{77.87}                     \\
%\hline
%\textcolor{blue}{\textbf{Mean Absolute Error of Lines of Code}} & \textcolor{blue}{0.84}           & \textcolor{blue}{8.89}                & \textcolor{blue}{3.05}           & \textcolor{blue}{11.95}                   & \textcolor{blue}{1.55}           & \textcolor{blue}{7.60}              & \textcolor{blue}{0.81}           & \textcolor{blue}{5.08}                 & \textcolor{blue}{1.56}          & \textcolor{blue}{8.38}                     \\
%\hline
%\textcolor{blue}{\textbf{Mean Absolute Error of AST Representation Length}} & \textcolor{blue}{281.45}           & \textcolor{blue}{1106.62}                & \textcolor{blue}{713.33}           & \textcolor{blue}{2545.19}                   & \textcolor{blue}{341.90}           & \textcolor{blue}{1433.30}              & \textcolor{blue}{241.67}           & \textcolor{blue}{912.85}                 & \textcolor{blue}{394.58}          & \textcolor{blue}{1225.60}                     \\
\hline
\end{tabular}
\end{adjustbox}
\end{table*}




==> todo.tex <==
TODO:

- Make rows blue -> DONE
- Add explanation for not conducting 2-3, 2-4 since the performance is different and generated from different models. Distance with human -> DONE
- Statistical analysis for Table VIII -> DONE
- Report size of code for Within vs Across (LOC, size of AST) -> DONE
- Write a paragraph in Discussion - for across experiment (This result is expected as this is observed in defect prediction ..) -> DONE

- Write new analysis in METHOD -> DONE
- Split paragraph from "The results ..." in Results.D -> DONE
- Add citations -> DONE
- Check Response letter


Through our analysis of prompt changes, we identified eight distinct categories of modifications that developers make when evolving their prompts (Table \ref{table:change-type-frequency}). These changes are categorized into component-dependent and component-independent modifications based on whether they target specific prompt components or affect the prompt's overall structure and presentation. Component-dependent changes, accounting for 64.4\% of all changes, directly affect specific components within prompts. Additions (30.1\%) emerge as the most frequent type, indicating that initial prompts often require expansion over time. Modifications (25.5\%) represent changes that alter the semantic meaning or behavior specification of existing components. While removals are also component-dependent, they occur less frequently (8.8\%), suggesting that developers typically expand and enhance their prompts rather than reduce them. Component-independent changes, comprising 34.5\% of modifications, affect the prompt's overall structure or presentation without targeting specific components. Rephrasing (17.4\%) is the most common in this category, following two main approaches: simplifying complex instructions or enhancing clarity through better expression. Formatting changes (7.9\%) focus on template and whitespace modifications, while corrections (4.9\%) address basic spelling and grammar issues. Generalization (2.3\%) and restructuring (2.0\%) are the least frequent, indicating that developers rarely make broad structural changes once a prompt's organization is established.

Prompt changes primarily target specific components through additions and modifications, while changes affecting the overall prompt structure or presentation occur less frequently and focus mainly on clarity improvements.

